IRAS 08544-4431 : a new post-AGB star in a binary system surrounded by a dusty disc

We present an analysis of our extensive data-set on IRAS 08544-4431. It is the first object we discuss of our newly defined sample of stars, selected for their position in the 'RV Tauri' box in the IRAS [12]-[25], [25]-[60] two-color diagram. Moreover, our selection criteria included an observed excess in the L-band, indicative of a dusty disc. The SED of IRAS 08544-4431 shows a broad IR excess starting already at H. Our optical photometric data reveal some evidence for deep and] shallow minima in the light curve and a pulsation time-scale of around 100 days with a small amplitude (peak-to-peak amplitude in V = 0.17 mag). Our CORALIE radial velocity measurements show that IRAS 08544-4431 is a binary system with a period of 499 +/- 3 days and a mass function of 0.02 M_sun. Moreover, IRAS 08544-4431 is detected in both the CO (2-1) and (1-0) mm-wave emission lines. The triangular shape of the weak CO profile confirms that part of the circumstellar material is not freely expanding but resides probably in a dusty circumbinary disc. Our chemical abundance analysis of a high resolution spectrum of high S/N reveals that a depletion process has modified the photospheric abundances to a moderate extent ([Zn/Fe]=+0.4). All these findings confirm that the F-type IRAS 08544-4431 is another good example of a binary Post-AGB star surrounded by a dusty disc. The H-alpha P-Cygni profile shows ongoing mass-loss with a very high outflow velocity, the origin of which is not understood. The strength and velocity of the H-alpha-absorption are modulated with the orbital motion; the maxima of both quantities (+/- 400 km/s, 5 Angstrom, respectively) occur at superior conjunction.

==> H4172aa <==
%% file: AAJOUR.BIB = journal strings, new AA & AoJ abbreviations
%% last: Oct 31 1995
%% baton: Rob Rutten, Sterrekundig Instituut Utrecht
%%     >> don't change this file - its baton is mine all the time <<

@STRING{acta = "Acta Astron."}
@STRING{actastsin = "Acta Astron.\ Sin."}
@STRING{actapsin = "Acta Astrophys.\ Sin."}
@STRING{advp = "Adv.\ Phys."}
@STRING{advsr = "Adv.\ Space Res."}
@STRING{amjp = "Am.\ J.\ Phys."}
@STRING{annap = "Ann.\ d'Astrophys."}
@STRING{annrev = "ARA\hbox{\rm \&}A"}
@STRING{araa = "ARA\hbox{\rm \&}A"}
@STRING{ao = "Appl.\ Opt."}
@STRING{appl = "Appl.\ Phys.\ Lett."}
@STRING{apb = "Appl.\ Phys.\ B"}
@STRING{afz = "Afz"}
@STRING{aa = "A\hbox{\rm \&}A"}
@STRING{aar = "A\hbox{\rm \&}AR"}
@STRING{aas = "A\hbox{\rm \&}AS"}
@STRING{agas = "Astron.\ Ges.\ Abstr.\ Ser."}
@STRING{aj = "AJ"}
@STRING{an = "Astron.\ Nachr."}
@STRING{azh = "AZh"}
@STRING{apj = "ApJ"}
@STRING{apjl = "ApJ"}
@STRING{apjss = "ApJS"}
@STRING{apss = "Ap\hbox{\rm \&}SS"}
@STRING{ap = "Astrophysics"}
@STRING{ajp = "Aust.\ J.\ Phys."}
@STRING{baas = "BAAS"}
@STRING{ban = "Bull.\ Astron.\ Inst.\ Neth."}
@STRING{bac = "Bull.\ Astron.\ Inst.\ Czech."}
@STRING{cjp = "Can.\ J.\ Phys."}
@STRING{cm = "Celest.\ Mech."}
@STRING{chinaa = "Chin.\ Astron."}
@STRING{cast = "Comments Astrophys."}
@STRING{fiz = "Fizika"}
@STRING{gafd = "Geophys.\ Astrophys.\ Fluid Dyn."}
@STRING{gj = "Geophys.\ J."}
@STRING{grl = "Geophys.\ Res.\ Lett."}
@STRING{geo = "Geophysics"}
@STRING{hd = "Hemel en Dampkring"}
@STRING{iauc = "IAU Circ."}
@STRING{iauib = "IAU Inf.\ Bull."}
@STRING{icarus = "Icarus"}
@STRING{jap = "J.\ Appl.\ Phys."}
@STRING{jaa = "JA\hbox{\rm \&}A"}
@STRING{jas = "J.\ Atmos.\ Sci."}
@STRING{jchemp = "J.\ Chem.\ Phys."}
@STRING{jcomp = "J.\ Comp.\ Phys."}
@STRING{jfm = "J.\ Fluid Mech."}
@STRING{jgr = "J.\ Geophys.\ Res."}
@STRING{jhast = "J.\ Hist.\ Astron."}
@STRING{jmolspec = "J.\ Mol.\ Spectrosc."}
@STRING{josa = "J.\ Opt.\ Soc.\ Am."}
@STRING{josaa = "J.\ Opt.\ Soc.\ Am.\ A"}
@STRING{josab = "J.\ Opt.\ Soc.\ Am.\ B"}
@STRING{jp = "J.\ Phys."}
@STRING{jpa = "J.\ Phys.\ A"}
@STRING{jpb = "J.\ Phys.\ B"}
@STRING{jpd = "J.\ Phys.\ D"}
@STRING{jpe = "J.\ Phys.\ E"}
@STRING{jpg = "J.\ Phys.\ G"}
@STRING{jpsj = "J.\ Phys.\ Soc.\ Japan"}
@STRING{jpp = "J.\ Plasma Phys."}
@STRING{jqsrt = "J.\ Quant.\ Spectrosc.\ Radiat.\ Transfer"}
@STRING{jrasc = "J.\ R.\ Astron.\ Soc.\ Can."}
@STRING{jetpl = "JETP Lett."}
@STRING{kfnt = "Kinematika Fiz.\ Nebesn.\ Tel"}
@STRING{msai = "Mem.\ Soc.\ Astron.\ Ital."}
@STRING{merc = "Mercury"}
@STRING{mag = "Mitt.\ Astron.\ Ges."}
@STRING{mn = "MNRAS"}
@STRING{mnras = "MNRAS"}
@STRING{mnassa = "Mon.\ Notes Astron.\ Soc.\ S.\ Afr."}
@STRING{nat = "Nat"}
@STRING{nature="Nat"}
@STRING{natwis = "Naturwissenschaften"}
@STRING{nattech = "Natuur en Techniek"}
@STRING{obs = "Observatory"}
@STRING{pfa = "Phys.\ Fluids A"}
@STRING{pfb = "Phys.\ Fluids B"}
@STRING{pla = "Phys.\ Lett.\ A"}
@STRING{plb = "Phys.\ Lett.\ B"}
@STRING{pra = "Phys.\ Rev.\ A"}
@STRING{prb = "Phys.\ Rev.\ B"}
@STRING{prc = "Phys.\ Rev.\ C"}
@STRING{prd = "Phys.\ Rev.\ D"}
@STRING{prl = "Phys.\ Rev.\ Lett."}
@STRING{ps = "Phys.\ Scr."}
@STRING{ptod = "Phys.\ Today"}
@STRING{pha = "Physica A"}
@STRING{phb = "Physica B"}
@STRING{phd = "Physica D"}
@STRING{pss = "Planet.\ Space Sci."}
@STRING{ppcf = "Plasma Phys.\ Controlled Fusion"}
@STRING{pasa = "Proc.\ Astron.\ Soc.\ Aust."}
@STRING{pi3e = "Proc.\ IEEE"}
@STRING{prsl = "Proc.\ R.\ Soc.\ London Ser.\ A"}
@STRING{posp = "Proceedings of SPIE"}
@STRING{pasj = "PASJ"}
@STRING{pasp = "PASP"}
@STRING{paspc = "PASPC"}
@STRING{qjras = "QJRAS"}
@STRING{ra = "Rev.\ Astron."}
@STRING{sciam = "Sci.\ Am."}
@STRING{sc = "Sci"}
@STRING{sky = "Sky Telesc."}
@STRING{sp = "Solar Phys."}
@STRING{sdb = "Soln.\ Dannye Byull."}
@STRING{sonne = "Sonne"}
@STRING{sa = "SvA"}
@STRING{sal = "SvA"}
@STRING{ssr = "Space Sci.\ Rev."}
@STRING{sf = "Spaceflight"}
@STRING{sterne = "Sterne"}
@STRING{sw = "Sterne Weltraum"}
@STRING{uao = "Upps.\ Astron.\ Obs.\ Rep."}
@STRING{va = "Vistas Astron."}
@STRING{zpa = "Z.\ Phys.\ A"}
@STRING{zpc = "Z.\ Phys.\ C"}
@STRING{zenit = "Zenit"}
@STRING{zetf = "Zh.\ Ehksp.\ Teor.\ Fiz."}
@STRING{ZsAp = "Zs.\ f.\ Ap."}
@STRING{ZsP = "Zs.\ f.\ Phys."}


==> H4172bib <==
@ARTICLE{1998AJ....115.1921A,
    author = {{Alcock}, C. and {Allsman}, R.~A. and {Alves}, D.~R. and {Axelrod}, T.~S. and 
        {Becker}, A. and {Bennett}, D.~P. and {Cook}, K.~H. and {Freeman}, K.~C. and 
        {Griest}, K. and {Lawson}, W.~A. and {Lehner}, M.~J. and {Marshall}, S.~L. and 
        {Minniti}, D. and {Peterson}, B.~A. and {Pollard}, K.~R. and 
        {Pratt}, M.~R. and {Quinn}, P.~J. and {Rodgers}, A.~W. and {Sutherland}, W. and 
        {Tomaney}, A. and {Welch}, D.~L.},
    title = "{The MACHO Project LMC Variable Star Inventory. VII. The Discovery of RV Tauri Stars and New Type II Cepheids in the Large Magellanic Cloud}",
    journal = {\aj},
    year = 1998,
    month = may,
    volume = 115,
    pages = {1921-1933},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998AJ....115.1921A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{1991A&A...245..499A,
    author = {{Alcolea}, J. and {Bujarrabal}, V.},
    title = "{The post-AGB evolution of low-mass stars}",
    journal = {\aap},
    year = 1991,
    month = may,
    volume = 245,
    pages = {499-512},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...245..499A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1995A&A...303L..21A,
    author = {{Alcolea}, J. and {Bujarrabal}, V.},
    title = "{The molecular envelope around 89 Herculis.}",
    journal = {\aap},
    year = 1995,
    month = nov,
    volume = 303,
    pages = {L21+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...303L..21A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1992A&A...258..104A,
    author = {{Arenou}, F. and {Grenon}, M. and {Gomez}, A.},
    title = "{A tridimensional model of the galactic interstellar extinction}",
    journal = {\aap},
    year = 1992,
    month = may,
    volume = 258,
    pages = {104-111},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...258..104A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1987ApJ...312..203B,
    author = {{Bond}, H.~E. and {Luck}, R.~E.},
    title = "{Nitrogen and sulfur overabundances in the population II supergiant HD 46703}",
    journal = {\apj},
    year = 1987,
    month = jan,
    volume = 312,
    pages = {203-210},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1987ApJ...312..203B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1988A&A...206L..17B,
    author = {{Bujarrabal}, V. and {Bachiller}, R. and {Alcolea}, J. and {Martin-Pintado}, J.
        },
    title = "{CO microwave emission from RV Tau variables}",
    journal = {\aap},
    year = 1988,
    month = nov,
    volume = 206,
    pages = {L17-L19},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988A%26A...206L..17B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1989ApJ...347..977B,
    author = {{Buss}, R.~H. and {Snow}, T.~P. and {Lamers}, H.~J.~G.~L.~M.
        },
    title = "{Grain ultraviolet extinction properties of recently discovered POST asymptotic giant branch stars}",
    journal = {\apj},
    year = 1989,
    month = dec,
    volume = 347,
    pages = {977-988},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989ApJ...347..977B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1993ApJ...412..431B,
    author = {{Bi{\'e}mont}, E. and {Hibbert}, A. and {Godefroid}, M. and {Vaeck}, N.
        },
    title = "{New f-values in C I and the CNO abundances in the sun}",
    journal = {\apj},
    year = 1993,
    month = jul,
    volume = 412,
    pages = {431-435},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJ...412..431B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1991ApJ...375..818B,
    author = {{Bi{\'e}mont}, E. and {Hibbert}, A. and {Godefroid}, M. and {Vaeck}, N. and 
        {Fawcett}, B.~C.},
    title = "{Accurate oscillator strengths of astrophysical interest for neutral oxygen}",
    journal = {\apj},
    year = 1991,
    month = jul,
    volume = 375,
    pages = {818-822},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991ApJ...375..818B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}




@ARTICLE{1990MNRAS.242....1C,
    author = {{Carter}, B.~S.},
    title = "{Southern JHKL standards}",
    journal = {\mnras},
    year = 1990,
    month = jan,
    volume = 242,
    pages = {1-5},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990MNRAS.242....1C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1905AN....168...29C,
    author = {{Ceraski}, W.},
    title = "{Trois nouvelles variables}",
    journal = {Astronomische Nachrichten},
    year = 1905,
    month = jul,
    volume = 168,
    pages = {29-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1905AN....168...29C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{debye,
    author ={{Chackerian}, C. and {Tipping}, R. H.},
    journal = {J. Mol. Spectrosc.},
    year = 1983,
    volume = 99,  
    pages ={431}
}

@ARTICLE{1996PASP..108..225C,
    author = {{Clayton}, G.~C.},
    title = "{The R Coronae Borealis Stars}",
    journal = {\pasp},
    year = 1996,
    month = mar,
    volume = 108,
    pages = {225-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996PASP..108..225C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2003A&A...397..595D,
    author = {{Dominik}, C. and {Dullemond}, C.~P. and {Cami}, J. and {van Winckel}, H.
        },
    title = "{The dust disk of HR 4049. Another brick in the wall}",
    journal = {\aap},
    year = 2003,
    month = jan,
    volume = 397,
    pages = {595-609},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2003A%26A...397..595D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1988ApJS...66..183E,
    author = {{Eder}, J. and {Lewis}, B.~M. and {Terzian}, Y.},
    title = "{New OH/IR stars from color-selected IRAS sources - 1612 MHz observations}",
    journal = {\apjs},
    year = 1988,
    month = feb,
    volume = 66,
    pages = {183-207},
    adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1988ApJS...66..183E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1999STIN...0014854E,
    author = {{Egan}, M.~P. and {Price}, S.~D. and {Moshir}, M.~M. and {Cohen}, M. and 
        {Tedesco}, E.},
    title = "{The Midcourse Space Experiment Point Source Catalog Version 1.2 Explanatory Guide}",
    journal = {Technical Report, AD-A381933; AFRL-VS-TR-1999-1522},
    year = 1999,
    month = jun,
    pages = {14854-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999STIN...0014854E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{1981ApJ...243..576F,
    author = {{Fernie}, J.~D.},
    title = "{89 Herculis - Further misdemeanors}",
    journal = {\apj},
    year = 1981,
    month = jan,
    volume = 243,
    pages = {576-582},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ApJ...243..576F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...469..355F,
    author = {{Flower}, P.~J.},
    title = "{Transformations from Theoretical Hertzsprung-Russell Diagrams to Color-Magnitude Diagrams: Effective Temperatures, B-V Colors, and Bolometric Corrections}",
    journal = {\apj},
    year = 1996,
    month = sep,
    volume = 469,
    pages = {355-+},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996ApJ...469..355F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1994A&A...292..133F,
    author = {{Fokin}, A.~B.},
    title = "{Nonlinear pulsations of the RV Tauri stars}",
    journal = {\aap},
    year = 1994,
    month = dec,
    volume = 292,
    pages = {133-151},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...292..133F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1972ApJ...178..715G,
    author = {{Gehrz}, R.~D.},
    title = "{Infrared Radiation from RV Tauri Stars. I. an Infrared Survey of RV Tauri Stars and Related Objects.}",
    journal = {\apj},
    year = 1972,
    month = dec,
    volume = 178,
    pages = {715-726},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1972ApJ...178..715G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1972PASP...84..768G,
    author = {{Gehrz}, R.~D. and {Ney}, E.~P.},
    title = "{Infrared Observations of Southern RV Tauri Stars}",
    journal = {\pasp},
    year = 1972,
    month = dec,
    volume = 84,
    pages = {768-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1972PASP...84..768G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1990A&A...237..159G,
    author = {{Gillet}, D. and {Burki}, G. and {Duquennoy}, A.},
    title = "{The pulsation of the photosphere of the RV Tauri stars - AC Herculis and R Scuti}",
    journal = {\aap},
    year = 1990,
    month = oct,
    volume = 237,
    pages = {159-168},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990A%26A...237..159G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1989A&A...215..316G,
    author = {{Gillet}, D. and {Duquennoy}, A. and {Bouchet}, P. and {Gouiffes}, C.
        },
    title = "{Shock phenomena in the atmosphere of the RV Tauri star, R Scuti}",
    journal = {\aap},
    year = 1989,
    month = may,
    volume = 215,
    pages = {316-330},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989A%26A...215..316G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1990Obs...110..120G,
    author = {{Giridhar}, S. and {Kameswara-Rao}, N. and {Lambert}, D.~L.},
    title = "{Is LR SCO and RCB star?}",
    journal = {The Observatory},
    year = 1990,
    month = aug,
    volume = 110,
    pages = {120-122},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990Obs...110..120G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1992JApA...13..307G,
    author = {{Giridhar}, S. and {Rao}, N.~K. and {Lambert}, D.~L.},
    title = "{High resolution spectroscopy of the semi-regular variable LR SCO}",
    journal = {Journal of Astrophysics and Astronomy},
    year = 1992,
    month = dec,
    volume = 13,
    pages = {307-318},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992JApA...13..307G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{1994ApJ...437..476G,
    author = {{Giridhar}, S. and {Rao}, N.~K. and {Lambert}, D.~L.},
    title = "{The chemical composition of the RV Tauri variable IW Carinae}",
    journal = {\apj},
    year = 1994,
    month = dec,
    volume = 437,
    pages = {476-484},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994ApJ...437..476G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...509..366G,
    author = {{Giridhar}, S. and {Lambert}, D.~L. and {Gonzalez}, G.},
    title = "{Abundance Analyses of Field RV Tauri Stars. IV. AD Aquilae, DS Aquarii, V360 Cygni, AC Herculis, and V453 Ophiuchi}",
    journal = {\apj},
    year = 1998,
    month = dec,
    volume = 509,
    pages = {366-378},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998ApJ...509..366G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...531..521G,
    author = {{Giridhar}, S. and {Lambert}, D.~L. and {Gonzalez}, G.},
    title = "{Abundance Analyses of Field RV Tauri Stars. V. DS Aquarii, UY Arae, TW Camelopardalis, BT Librae, U Monocerotis, TT Ophiuchi, R Scuti, and RV Tauri}",
    journal = {\apj},
    year = 2000,
    month = mar,
    volume = 531,
    pages = {521-536},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000ApJ...531..521G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1999MNSSA..58..147G,
    author = {{Glass}, I.~S.},
    title = "{PICNIC Near Infrared Camera}",
    journal = {Monthly Notes of the Astron.~Soc.~Southern Africa, Vol.~58, p.~147},
    year = 1999,
    volume = 58,
    pages = {147-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999MNSSA..58..147G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2002MNRAS.332L..55G,
    author = {{Gledhill}, T.~M. and {Bains}, I. and {Yates}, J.~A.},
    title = "{Submillimetre photometry of post-asymptotic giant branch stars}",
    journal = {\mnras},
    year = 2002,
    month = may,
    volume = 332,
    pages = {L55-L58},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002MNRAS.332L..55G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{2001MNRAS.322..321G,
    author = {{Gledhill}, T.~M. and {Chrysostomou}, A. and {Hough}, J.~H. and 
        {Yates}, J.~A.},
    title = "{Axisymmetry in protoplanetary nebulae: using imaging polarimetry to investigate envelope structure}",
    journal = {\mnras},
    year = 2001,
    month = apr,
    volume = 322,
    pages = {321-342},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001MNRAS.322..321G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1990RMxAA..20...55G,
    author = {{Gomez}, Y. and {Moran}, J.~M. and {Rodriguez}, L.~F.},
    title = "{H2O and SiO maser emission in OH/IR stars.}",
    journal = {Revista Mexicana de Astronomia y Astrofisica},
    year = 1990,
    month = jun,
    volume = 20,
    pages = {55-+},
    adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1990RMxAA..20...55G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1997ApJ...479..427G,
    author = {{Gonzalez}, G. and {Lambert}, D.~L. and {Giridhar}, S.},
    title = "{Abundance Analyses of the Field RV Tauri Variables: EP Lyrae, DY Orionis, AR Puppis, and R Sagittae}",
    journal = {\apj},
    year = 1997,
    month = apr,
    volume = 479,
    pages = {427-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997ApJ...479..427G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1997ApJ...481..452G,
    author = {{Gonzalez}, G. and {Lambert}, D.~L. and {Giridhar}, S.},
    title = "{Abundance Analyses of Field RV Tauri Variables. III. DY Aquilae, SS Geminorum, CT Orionis, and CE Virginis}",
    journal = {\apj},
    year = 1997,
    month = may,
    volume = 481,
    pages = {452-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997ApJ...481..452G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{1998SSRv...85..161G,
    author = {{Grevesse}, N. and {Sauval}, A.~J.},
    title = "{Standard Solar Composition}",
    journal = {Space Science Reviews},
    year = 1998,
    month = aug,
    volume = 85,
    pages = {161-174},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998SSRv...85..161G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2002A&A...390..501G,
    author = {{Groenewegen}, M.~A.~T. and {Sevenster}, M. and {Spoon}, H.~W.~W. and 
        {P{\' e}rez}, I.},
    title = "{Millimetre observations of infrared carbon stars. I. The data}",
    journal = {\aap},
    year = 2002,
    month = aug,
    volume = 390,
    pages = {501-510},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002A%26A...390..501G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1991A&AS...90..327T,
    author = {{Te Lintel Hekkert}, P. and {Caswell}, J.~L. and {Habing}, H.~J. and 
        {Haynes}, R.~F. and {Haynes}, R.~F. and {Norris}, R.~P.},
    title = "{1612 MHz OH survey of IRAS point sources. I - Observations made at Dwingeloo, Effelsberg and Parkes}",
    journal = {\aaps},
    year = 1991,
    month = oct,
    volume = 90,
    pages = {327-353},
    adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1991A%26AS...90..327T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1991A&AS...88..505H,
    author = {{Hibbert}, A. and {Biemont}, E. and {Godefroid}, M. and {Vaeck}, N.
        },
    title = "{New accurate transition probabilities for astrophysically important spectral lines of neutral nitrogen}",
    journal = {\aaps},
    year = 1991,
    month = jun,
    volume = 88,
    pages = {505-524},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26AS...88..505H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{2001sgc..conf...23H,
    author = {{Holweger}, H.},
    title = "{Photospheric Abundances: Problems, Updates, Implications}",
    booktitle = {AIP Conf. Proc. 598: Joint SOHO/ACE workshop "Solar and Galactic Composition"},
    year = 2001,
    pages = {23-+},
    EDITOR    = {{Wimmer-Schweingruber}, R.~F.}, 
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001sgc..conf...23H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1999MNRAS.306..531J,
    author = {{Johnson}, J.~J. and {Anderson}, C.~M. and {Bjorkman}, K.~S. and 
        {Code}, A.~D. and {Fox}, G.~K. and {Weitenbeck}, A.~J. and {Babler}, B.~L. and 
        {Meade}, M.~R. and {Zellner}, N.~E.~B. and {Lupie}, O.~L.},
    title = "{HR 4049: temporal variations in the structure of the circumstellar material}",
    journal = {\mnras},
    year = 1999,
    month = jul,
    volume = 306,
    pages = {531-537},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999MNRAS.306..531J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1987A&A...181...31J,
    author = {{Joshi}, U.~C. and {Deshpande}, M.~R. and {Sen}, A.~K. and {Kulshrestha}, A.
        },
    title = "{Polarization investigations in four peculiar supergiants with high IR excess}",
    journal = {\aap},
    year = 1987,
    month = jul,
    volume = 181,
    pages = {31-33},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1987A%26A...181...31J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{1982SPIE..331..368J,
    author = {{Jorden}, A.~R. and {Read}, P.~D. and {van Breda}, I.~G.},
    title = "{Photon Counting RETICON System - Description and Performance}",
    booktitle = {INSTRUMENTATION IN ASTRONOMY IV: TUCSON: SPIE331 P.368, 1982},
    year = 1982,
    volume = 331,
    pages = {368-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982SPIE..331..368J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...521..302J,
    author = {{Jura}, M. and {Kahane}, C.},
    title = "{Orbiting Molecular Reservoirs around Evolved Red Giant Stars}",
    journal = {\apj},
    year = 1999,
    month = aug,
    volume = 521,
    pages = {302-309},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999ApJ...521..302J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1997ApJ...485..341J,
    author = {{Jura}, M. and {Kahane}, C. and {Fischer}, D. and {Grady}, C.
        },
    title = "{Circumstellar Gas in the Wide Binary HD 188037}",
    journal = {\apj},
    year = 1997,
    month = aug,
    volume = 485,
    pages = {341-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997ApJ...485..341J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1995ApJ...453..721J,
    author = {{Jura}, M. and {Balm}, S.~P. and {Kahane}, C.},
    title = "{A Long-lived Disk around the Red Rectangle?}",
    journal = {\apj},
    year = 1995,
    month = nov,
    volume = 453,
    pages = {721-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995ApJ...453..721J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...541..264J,
    author = {{Jura}, M. and {Chen}, C. and {Werner}, M.~W.},
    title = "{The Dust Ring around AC Herculis}",
    journal = {\apj},
    year = 2000,
    month = sep,
    volume = 541,
    pages = {264-269},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000ApJ...541..264J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1998ApJ...500..466K,
    author = {{Kahane}, C. and {Barnbaum}, C. and {Uchida}, K. and {Balm}, S.~P. and 
        {Jura}, M.},
    title = "{A Circumbinary Reservoir around BM Geminorum?}",
    journal = {\apj},
    year = 1998,
    month = jun,
    volume = 500,
    pages = {466-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998ApJ...500..466K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2002MNRAS.334..129K,
    author = {{Kameswara Rao}, N. and {Goswami}, A. and {Lambert}, D.~L.},
    title = "{High-resolution spectroscopy of QY Sge: an obscured RV Tauri variable?}",
    journal = {\mnras},
    year = 2002,
    month = jul,
    volume = 334,
    pages = {129-136},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002MNRAS.334..129K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{2000MNRAS.316..689K,
    author = {{Karakas}, A.~I. and {Tout}, C.~A. and {Lattanzio}, J.~C.},
    title = "{The eccentricities of the barium stars}",
    journal = {\mnras},
    year = 2000,
    month = aug,
    volume = 316,
    pages = {689-698},
    url =
{http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2000MNRAS.316..689K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2001IBVS.5135....1K,
    author = {{Kazarovets}, E.~V. and {Samus}, N.~N. and {Durlevich}, O.~V.
        },
    title = "{The 76th Name-List of Variable Stars}",
    journal = {Informational Bulletin on Variable Stars},
    year = 2001,
    month = jul,
    volume = 5135,
    pages = {1-+},
    adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=2001IBVS.5135....1K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2001ARep...45..553K,
    author = {{Klochkova}, V.~G. and {Zhao}, G. and {Panchuk}, V.~E. and {Tavolganskaya}, N.~S.
        },
    title = "{Optical Spectra of Three AGB Stars}",
    journal = {Astronomy Reports},
    year = 2001,
    month = jul,
    volume = 45,
    pages = {553-563},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001ARep...45..553K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1970ApJ...159..485K,
    author = {{Kodaira}, K. and {Greenstein}, J.~L. and {Oke}, J.~B.},
    title = "{The Unusual Composition of +39{\deg}4926}",
    journal = {\apj},
    year = 1970,
    month = feb,
    volume = 159,
    pages = {485-+},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1970ApJ...159..485K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1973A&A....22..273K,
    author = {{Kodaira}, K.},
    title = "{Revised chemical abundances of four population-II A-type stars.}",
    journal = {\aap},
    year = 1973,
    month = jan,
    volume = 22,
    pages = {273-279},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1973A%26A....22..273K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2002ApJS..140..389K,
    author = {{Kraemer}, K.~E. and {Sloan}, G.~C. and {Price}, S.~D. and {Walker}, H.~J.
        },
    title = "{Classification of 2.4-45.2 Micron Spectra from the Infrared Space Observatory Short Wavelength Spectrometer}",
    journal = {\apjs},
    year = 2002,
    month = jun,
    volume = 140,
    pages = {389-406},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002ApJS..140..389K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1999A&A...347..235K,
    author = {{Kre{\l}owski}, J. and {Ehrenfreund}, P. and {Foing}, B.~H. and 
        {Snow}, T.~P. and {Weselak}, T. and {Tuairisg}, S.~{\' O}. and 
        {Galazutdinov}, G.~A. and {Musaev}, F.~A.},
    title = "{On the relation between diffuse interstellar bands and simple molecular species}",
    journal = {\aap},
    year = 1999,
    month = jul,
    volume = 347,
    pages = {235-242},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...347..235K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{1971GCVS3.C......0K,
    author = {{Kukarkin}, B.~V. and {Kholopov}, P.~N. and {Pskovsky}, Y.~P. and 
        {Efremov}, Y.~N. and {Kukarkina}, N.~P. and {Kurochkin}, N.~E. and 
        {Medvedeva}, G.~I.},
    title = "{The third edition containing information on 20437 variable stars discovered and designated till 1968.}",
    booktitle = {General Catalogue of Variable Stars, 3rd ed. (1971)},
    year = 1971,
    pages = {0-+},
    adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1971GCVS3.C......0K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1982ApJ...263..226K,
    author = {{Kunasz}, P.~B. and {Morrison}, N.~D.},
    title = "{Mass loss in Alpha Cygni - Synthetic H-Alpha profiles}",
    journal = {\apj},
    year = 1982,
    month = dec,
    volume = 263,
    pages = {226-238},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982ApJ...263..226K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1999A&AS..138..119K,
    author = {{Kupka}, F. and {Piskunov}, N. and {Ryabchikova}, T.~A. and 
        {Stempels}, H.~C. and {Weiss}, W.~W.},
    title = "{VALD-2: Progress of the Vienna Atomic Line Data Base}",
    journal = {\aaps},
    year = 1999,
    month = jul,
    volume = 138,
    pages = {119-133},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26AS..138..119K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1993KurCD..13.....K,
    author = {{Kurucz}, R.},
    title = "{ATLAS9 Stellar Atmosphere Programs and 2 km/s grid.}",
    journal = {ATLAS9 Stellar Atmosphere Programs and 2 km/s grid.~Kurucz CD-ROM No.~13.~ Cambridge, Mass.: Smithsonian Astrophysical Observatory, 1993.},
    year = 1993,
    volume = 13,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993KurCD..13.....K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1997ApJS..112..557K,
    author = {{Kwok}, S. and {Volk}, K. and {Bidelman}, W.~P.},
    title = "{Classification and Identification of IRAS Sources with Low-Resolution Spectra}",
    journal = {\apjs},
    year = 1997,
    month = oct,
    volume = 112,
    pages = {557-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997ApJS..112..557K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1988ApJ...333..917L,
    author = {{Lambert}, D.~L. and {Hinkle}, K.~H. and {Luck}, R.~E.},
    title = "{The peculiar supergiant HR 4049}",
    journal = {\apj},
    year = 1988,
    month = oct,
    volume = 333,
    pages = {917-924},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988ApJ...333..917L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
} 
 
@ARTICLE{1986A&A...154L..20L,
    author = {{Lamers}, H.~J.~G.~L.~M. and {Waters}, L.~B.~F.~M. and {Garmany}, C.~D. and 
        {Perez}, M.~R. and {Waelkens}, C.},
    title = "{HR 4049 - The hottest proto-planetary nebula star or a run-away hypergiant at high galactic latitude surrounded by a dust cloud?}",
    journal = {\aap},
    year = 1986,
    month = jan,
    volume = 154,
    pages = {L20-L22},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...154L..20L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}
 
 

@BOOK{Lodders,
    author = {{Lodders}, K. and {Fegley}, B.}, 
    title = "{The Planetary Scientist's Companion}",
    year= 1988,
    publisher =  {Oxford University Press},
    pages = {83},
}

@ARTICLE{1991A&A...246..490L,
    author = {{L{\` e}bre}, A. and {Gillet}, D.},
    title = "{The bright RV Tauri star R Scuti during an exceptional irregular light phase}",
    journal = {\aap},
    year = 1991,
    month = jun,
    volume = 246,
    pages = {490-502},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...246..490L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1991A&A...246..153L,
    author = {{Likkel}, L. and {Forveille}, T. and {Omont}, A. and {Morris}, M.
        },
    title = "{CO observations of cold IRAS objects - AGB and post-AGB stars}",
    journal = {\aap},
    year = 1991,
    month = jun,
    volume = 246,
    pages = {153-174},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...246..153L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1985MNRAS.217..493E,
    author = {{Lloyd Evans}, T.},
    title = "{Circumstellar material and the light variations of RV Tauri stars}",
    journal = {\mnras},
    year = 1985,
    month = nov,
    volume = 217,
    pages = {493-506},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985MNRAS.217..493E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1990MNRAS.243..336E,
    author = {{Lloyd Evans}, T.},
    title = "{Carbon stars with silicate dust shells. I - Carbon stars with enhanced C-13 (J stars)}",
    journal = {\mnras},
    year = 1990,
    month = mar,
    volume = 243,
    pages = {336-348},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990MNRAS.243..336E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{1997Ap&SS.251..239L,
    author = {{Lloyd Evans}, T.},
    title = "{Stars with Cool Dusty Disks}",
    journal = {\apss},
    year = 1997,
    volume = 251,
    pages = {239-242},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997Ap%26SS.251..239L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{1999IAUS..191..453E,
    author = {{Lloyd Evans}, T.},
    title = "{The Nature of RV Tauri Stars}",
    booktitle = {IAU Symp. 191: Asymptotic Giant Branch Stars},
    year = 1999,
    volume = 191,
    pages = {453-+},
    EDITOR    = {{Le Bertre}, T. and {L{\` e}bre}, A. and {Waelkens}, C.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999IAUS..191..453E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@INPROCEEDINGS{1992bats.proc..145L,
    author = {{Lubow}, S.~H. and {Artymowicz}, P.},
    title = "{Eccentricity Evolution of a Binary Embedded in a Disk}",
    booktitle = {Binaries as Tracers of Stellar Formation. Proceedings of a Workshop held in Bettmeralp, Switzerland, Sept. 1991, in honor of Dr. Roger Griffin. Editors, Antoine Duquennoy, Michel Mayor; Publisher, Cambridge University Press, Cambridge, England, New York, NY, 1992. LC \# QB821 .B55 1991. ISBN \# 0521433584. P. 145, 1992},
    year = 1992,
    pages = {145-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992bats.proc..145L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1984ApJ...279..729L,
    author = {{Luck}, R.~E. and {Bond}, H.~E.},
    title = "{HD 46703 - A high-luminosity population II F-type star}",
    journal = {\apj},
    year = 1984,
    month = apr,
    volume = 279,
    pages = {729-737},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984ApJ...279..729L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1990ApJ...357..188L,
    author = {{Luck}, R.~E. and {Bond}, H.~E. and {Lambert}, D.~L.},
    title = "{Chemical compositions of four high-latitude A-F supergiants}",
    journal = {\apj},
    year = 1990,
    month = jul,
    volume = 357,
    pages = {188-203},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJ...357..188L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1971AJ.....76..544L,
    author = {{Lucy}, L.~B. and {Sweeney}, M.~A.},
    title = "{Spectroscopic binaries with circular orbits.}",
    journal = {\aj},
    year = 1971,
    month = aug,
    volume = 76,
    pages = {544-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1971AJ.....76..544L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{2002A&A...386..504M,
    author = {{Maas}, T. and {Van Winckel}, H. and {Waelkens}, C.
        },
    title = "{RU Cen and SX Cen: Two strongly depleted RV Tauri stars in binary systems. The RV Tauri photometric b phenomenon and binarity}",
    journal = {\aap},
    year = 2002,
    month = may,
    volume = 386,
    pages = {504-516},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002A%26A...386..504M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2002MNSSA..61..102M,
    author = {{Martinez}, P. and {Kilkenny}, D.~M. and {Cox}, G. and {Carter}, D.~B. and 
        {Ellis}, D.~T. and {Evans}, G.~P. and {Fouche}, M. and {Koorts}, W.~P. and 
        {Metcalfe}, D. and {Pearson}, W. and {Riddick}, A. and {Sommeregger}, E. and 
        {Stoffels}, J. and {Weir}, D. and {Woodhouse}, G.},
    title = "{The automatic photometric telescope at the South African Astronomical Observatory.}",
    journal = {Monthly Notes of the Astronomical Society of South Africa},
    year = 2002,
    volume = 61,
    pages = {102-111},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002MNSSA..61..102M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1992A&A...259L..39M,
    author = {{Mathis}, J.~S. and {Lamers}, H.~J.~G.~L.~M.},
    title = "{The origin of the extremely metal-poor post-AGB stars}",
    journal = {\aap},
    year = 1992,
    month = jun,
    volume = 259,
    pages = {L39-L42},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...259L..39M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1988MNRAS.233..697M,
    author = {{Menzies}, J.~W. and {Whitelock}, P.~A.},
    title = "{IRAS 20056+1834 - A G star reflects on its past}",
    journal = {\mnras},
    year = 1988,
    month = aug,
    volume = 233,
    pages = {697-703},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988MNRAS.233..697M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1989SAAOC..13....1M,
    author = {{Menzies}, J.~W. and {Cousins}, A.~W.~J. and {Banfield}, R.~M. and 
        {Laing}, J.~D.},
    title = "{UBV (RI)c standard stars in the E- and F-regions and in the Magellanic Clouds - a revised catalogue.}",
    journal = {South African Astronomical Observatory Circular},
    year = 1989,
    volume = 13,
    pages = {1-13},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989SAAOC..13....1M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}
@ARTICLE{1999A&A...350..163M,
    author = {{Molster}, F.~J. and {Waters}, L.~B.~F.~M. and {Trams}, N.~R. and 
        {Van Winckel}, H. and {Decin}, L. and {van Loon}, J.~T. and 
        {J{\" a}ger}, C. and {Henning}, T. and {K{\" a}ufl}, H.-U. and 
        {de Koter}, A. and {Bouwman}, J.},
    title = "{The composition and nature of the dust shell surrounding the binary AFGL 4106}",
    journal = {\aap},
    year = 1999,
    month = oct,
    volume = 350,
    pages = {163-180},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...350..163M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1992A&AS...93..121N,
    author = {{Nyman}, L.-A. and {Booth}, R.~S. and {Carlstrom}, U. and {Habing}, H.~J. and 
        {Heske}, A. and {Sahai}, R. and {Stark}, R. and {van der Veen}, W.~E.~J.~C. and 
        {Winnberg}, A.},
    title = "{A survey of circumstellar CO emission from a sample of IRAS point sources}",
    journal = {\aaps},
    year = 1992,
    month = apr,
    volume = 93,
    pages = {121-150},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26AS...93..121N&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1993ApJS...87..267O,
    author = {{Olofsson}, H. and {Eriksson}, K. and {Gustafsson}, B. and {Carlstrom}, U.
        },
    title = "{A study of circumstellar envelopes around bright carbon stars. I - Structure, kinematics, and mass-loss rate.}",
    journal = {\apjs},
    year = 1993,
    month = jul,
    volume = 87,
    pages = {267-304},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJS...87..267O&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1986A&AS...65..607O,
    author = {{Olnon}, F.~M. and {Raimond}, E. and {Neugebauer}, G. and {van Duinen}, R.~J. and 
        {Habing}, H.~J. and {Aumann}, H.~H. and {Beintema}, D.~A. and 
        {Boggess}, N. and {Borgman}, J. and {Clegg}, P.~E. and {Gillett}, F.~C. and 
        {Hauser}, M.~G. and {Houck}, J.~R. and {Jennings}, R.~E. and 
        {de Jong}, T. and {Low}, F.~J. and {Marsden}, P.~L. and {Pottasch}, S.~R. and 
        {Soifer}, B.~T. and {Walker}, R.~G. and {Emerson}, J.~P. and 
        {Rowan-Robinson}, M. and {Wesselius}, P.~R. and {Baud}, B. and 
        {Beichman}, C.~A. and {Gautier}, T.~N. and {Harris}, S. and 
        {Miley}, G.~K. and {Young}, E.},
    title = "{IRAS catalogues and atlases - Atlas of low-resolution spectra}",
    journal = {\aaps},
    year = 1986,
    month = sep,
    volume = 65,
    pages = {607-1065},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26AS...65..607O&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2000A&AS..145..269P,
    author = {{Parthasarathy}, M. and {Vijapurkar}, J. and {Drilling}, J.~S.
        },
    title = "{Low resolution spectroscopy of hot post-AGB candidates}",
    journal = {\aaps},
    year = 2000,
    month = aug,
    volume = 145,
    pages = {269-274},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26AS..145..269P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}




@INPROCEEDINGS{1999psrv.conf...13Q,
    author = {{Queloz}, D. and {Casse}, M. and {Mayor}, M.},
    title = "{The Fiber-Fed Spectrograph, a Tool to Detect Planets}",
    booktitle = {ASP Conf. Ser. 185: IAU Colloq. 170: Precise Stellar Radial Velocities},
    year = 1999,
    pages = {13-+},
    EDITOR = {{Hearnshaw}, J.~B. and {Scarfe}, C.~D.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999psrv.conf...13Q&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1996MNRAS.279..949P,
    author = {{Pollard}, K.~R. and {Cottrell}, P.~L. and {Kilmartin}, P.~M. and 
        {Gilmore}, A.~C.},
    title = "{RV Tauri stars - I. A long-term photometric survey.}",
    journal = {\mnras},
    year = 1996,
    month = apr,
    volume = 279,
    pages = {949-977},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996MNRAS.279..949P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{pols2003,
    author = {{Pols}, O.R. and {Karakas}, A.I. and {Lattanzio}, J.C. {Tout} C.A.},
    title = "{}",
    booktitle = {Symbiotic stars probing stellar evolution},
    year = 2003,
    pages = {in press},
    EDITOR = {{Hack}, M.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1969mlfs.conf...57S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1963ApJ...137..401P,
    author = {{Preston}, G.~W. and {Krzeminski}, W. and {Smak}, J. and {Williams}, J.~A.
        },
    title = "{A Spectroscopic and Photoelectric Survey of the RV Tauri Stars.}",
    journal = {\apj},
    year = 1963,
    month = feb,
    volume = 137,
    pages = {401-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1963ApJ...137..401P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1996AAS...189.5102P,
    author = {{Price}, S.~D. and {Tedesco}, E.~F. and {Cohen}, M. and {Walker}, R.~G. and 
        {Henry}, R.~C. and {Moshir}, M. and {Paxton}, L.~J. and {Witteborn}, F.~C. and 
        {Egan}, M.~P. and {Shipman}, R.~F.},
    title = "{Astronomy on the Midcourse Space Experiment}",
    journal = {Bulletin of the American Astronomical Society},
    year = 1996,
    month = dec,
    volume = 28,
    pages = {1341-+},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996AAS...189.5102P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1989MNRAS.238..945R,
    author = {{Raveendran}, A.~V.},
    title = "{Dust envelopes around RV Tauri stars}",
    journal = {\mnras},
    year = 1989,
    month = jun,
    volume = 238,
    pages = {945-953},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989MNRAS.238..945R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Reyniers2002,
    author = {{Reyniers}, M.}, 
    title = "{High Resolution Spectroscopy of Post-AGB stars : AGB Nucleosynthesis
     and Dredge-up.}",
    year= 2002,
    publisher =  {KULEUVEN},
    pages = {},
}

@INPROCEEDINGS{1969mlfs.conf...57S,
    author = {{Sargent}, W.~L.~W. and {Osmer}, P.~S.},
    title = "{Evidence for Mass Loss from the F-Type Supergiant, 89 Herculis}",
    booktitle = {Mass Loss from Stars, Proceedings of the second Trieste Colloquium on Astrophysics},
    year = 1969,
    pages = {57-+},
    EDITOR = {{Hack}, M.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1969mlfs.conf...57S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1979ARA&A..17...73S,
    author = {{Savage}, B.~D. and {Mathis}, J.~S.},
    title = "{Observed properties of interstellar dust}",
    journal = {\araa},
    year = 1979,
    volume = 17,
    pages = {73-111},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ARA%26A..17...73S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1982ApJ...263..835S,
    author = {{Scargle}, J.~D.},
    title = "{Studies in astronomical time series analysis. II - Statistical aspects of spectral analysis of unevenly spaced data}",
    journal = {\apj},
    year = 1982,
    month = dec,
    volume = 263,
    pages = {835-853},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982ApJ...263..835S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1908LawOB...1..215S,
    author = {{Seares}, F.~H.},
    title = "{The Variable RV Tauri (45.1905)}",
    journal = {Laws Observatory Bulletin, University of Missouri},
    year = 1908,
    month = mar,
    volume = 1,
    pages = {215-222},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1908LawOB...1..215S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{1995MNRAS.273..906S,
    author = {{Shenton}, M. and {Evans}, A. and {Williams}, P.~M.},
    title = "{Millimetre continuum observations of low-mass carbon-rich stars}",
    journal = {\mnras},
    year = 1995,
    month = apr,
    volume = 273,
    pages = {906-912},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995MNRAS.273..906S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1978ApJ...224..953S,
    author = {{Stellingwerf}, R.~F.},
    title = "{Period determination using phase dispersion minimization}",
    journal = {\apj},
    year = 1978,
    month = sep,
    volume = 224,
    pages = {953-960},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978ApJ...224..953S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1978IBVS.1453....1S,
    author = {{Stephenson}, C.~B.},
    title = "{Spectral Information on Variable Stars}",
    journal = {Informational Bulletin on Variable Stars},
    year = 1978,
    volume = 1453,
    pages = {1-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978IBVS.1453....1S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2002PASJ...54..765T,
    author = {{Takeda}, Y. and {Parthasarathy}, M. and {Aoki}, W. and {Ita}, Y. and 
        {Nakada}, Y. and {Izumiura}, H. and {Noguchi}, K. and {Takada-Hidai}, M. and 
        {Sato}, B. and {Tajitsu}, A. and {Honda}, S. and {Kawanomoto}, S. and 
        {Ando}, H. and {Karoji}, H.},
    title = "{Detection of Zinc in the Very Metal-Poor Post-AGB Star HR 4049}",
    journal = {\pasj},
    year = 2002,
    month = oct,
    volume = 54,
    pages = {765-773},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2002PASJ...54..765T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{1994A&A...285..551V,
    author = {{van der Veen}, W.~E.~C.~J. and {Waters}, L.~B.~F.~M. and {Trams}, N.~R. and 
        {Matthews}, H.~E.},
    title = "{A study of dust shells around high latitude supergiants}",
    journal = {\aap},
    year = 1994,
    month = may,
    volume = 285,
    pages = {551-564},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...285..551V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{udry,
    author = {{Udry}, S. and {Mayor}, M.},
    booktitle = "{Astrobiology. The Quest for the conditions of life, ed. G. Horneck, \& C. Baumstark-Khan (Springer Verlag)}",
    year = 2001,
    pages = {25}, 
}

@ARTICLE{1994AJ....108..984T,
    author = {{Trammell}, S.~R. and {Dinerstein}, H.~L. and {Goodrich}, R.~W.
        },
    title = "{Evidence for the early onset of aspherical structure in the planetary nebula formation process: Spectropolarimetry of post-AGB stars}",
    journal = {\aj},
    year = 1994,
    month = sep,
    volume = 108,
    pages = {984-997},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994AJ....108..984T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{1995A&A...293L..25V,
    author = {{Van Winckel}, H. and {Waelkens}, C. and {Waters}, L.~B.~F.~M.
        },
    title = "{The extremely iron-deficient "Post-AGB" stars and binaries.}",
    journal = {\aap},
    year = 1995,
    month = jan,
    volume = 293,
    pages = {L25-L28},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...293L..25V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1998A&A...336L..17V,
    author = {{Van Winckel}, H. and {Waelkens}, C. and {Waters}, L.~B.~F.~M. and 
        {Molster}, F.~J. and {Udry}, S. and {Bakker}, E.~J.},
    title = "{The binary RV Tauri star AC HER and evidence for a long-lived dust-disc}",
    journal = {\aap},
    year = 1998,
    month = aug,
    volume = 336,
    pages = {L17-LL20},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...336L..17V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1999A&A...343..202V,
    author = {{Van Winckel}, H. and {Waelkens}, C. and {Fernie}, J.~D. and 
        {Waters}, L.~B.~F.~M.},
    title = "{The RV$\backslash$ Tauri phenomenon and binarity}",
    journal = {\aap},
    year = 1999,
    month = mar,
    volume = 343,
    pages = {202-212},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...343..202V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{2000A&A...354..135V,
    author = {{Van Winckel}, H. and {Reyniers}, M.},
    title = "{A homogeneous study of the s-process in the 21 mu m carbon-rich post-AGB objects}",
    journal = {\aap},
    year = 2000,
    month = feb,
    volume = 354,
    pages = {135-149},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26A...354..135V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{2001Ap&SS.275..159V,
    author = {{Van Winckel}, H.},
    title = "{Binary (Post) AGB evolution}",
    journal = {\apss},
    year = 2001,
    month = jan,
    volume = 275,
    pages = {159-167},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001Ap%26SS.275..159V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROOCEEDINGS{hansthesis,
    author = {{Van Winckel}, H.},
    title = "{Ph.D. thesis}",
    booktitle = {The chemical composition of optically bright post-AGB stars},
    year = 1995,
    volume = 3,
    pages = {1},
    EDITOR    = {a},
    url = {d},
    adsnote = {d}
}


@ARTICLE{1989A&A...211..208W,
    author = {{Waters}, L.~B.~F.~M. and {Lamers}, H.~J.~G.~L.~M. and {Snow}, T.~P. and 
        {Mathlener}, E. and {Trams}, N.~R. and {van Hoof}, P.~A.~M. and 
        {Waelkens}, C. and {Seab}, C.~G. and {Stanga}, R.},
    title = "{Circumstellar dust around HR 4049 - A critical test for theories of interstellar dust}",
    journal = {\aap},
    year = 1989,
    month = feb,
    volume = 211,
    pages = {208-216},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989A%26A...211..208W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
} 

@ARTICLE{1992A&A...262L..37W,
    author = {{Waters}, L.~B.~F.~M. and {Trams}, N.~R. and {Waelkens}, C.},
    title = "{A scenario for the selective depletion of stellar atmospheres}",
    journal = {\aap},
    year = 1992,
    month = sep,
    volume = 262,
    pages = {L37-L40},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...262L..37W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{1993A&A...269..242W,
    author = {{Waters}, L.~B.~F.~M. and {Waelkens}, C. and {Mayor}, M. and 
        {Trams}, N.~R.},
    title = "{A model for the 89 Herculis system}",
    journal = {\aap},
    year = 1993,
    month = mar,
    volume = 269,
    pages = {242-248},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...269..242W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{1997IAUS..180..313W,
    author = {{Waters}, L.B.F.M and {Waelkens}, C. and {Van Wickel}, H.},
    title = "{Binary Post-AGB stars}",
    booktitle = {IAU Symp. 180: Planetary Nebulae},
    year = 1997,
    volume = 180,
    pages = {313-+},
    EDITOR    = {{Habing}, H.J. and {Lamers}, H.J.G.L.M.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997IAUS..180..313W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1998Natur.391..868W,
    author = {{Waters}, L.~B.~F.~M. and {Cami}, J. and {de Jong}, T. and {Molster}, F.~J. and 
        {van Loon}, J.~T. and {Bouwman}, J. and {de Koter}, A. and {Waelkens}, C. and 
        {Van Winckel}, H. and {Morris}, P.~W.},
    title = "{An oxygen-rich dust disk surrounding an evolved star in the Red Rectangle}",
    journal = {\nat},
    year = 1998,
    month = feb,
    volume = 391,
    pages = {868-+},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998Natur.391..868W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{vanwinckel2003,
    author = {{Van Winckel}, H.},
    title = "{}",
    journal = {\araa},
    year = 2003,
    volume = 1,
    pages = {in press},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1987A&A...181L...5W,
    author = {{Waelkens}, C. and {Waters}, L.~B.~F.~M. and {Cassatella}, A. and 
        {Le Bertre}, T. and {Lamers}, H.~J.~G.~L.~M.},
    title = "{HD 213985 - A hot post-AGB star in the Galactic halo}",
    journal = {\aap},
    year = 1987,
    month = jul,
    volume = 181,
    pages = {L5-L8},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1987A%26A...181L...5W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1991A&A...242..433W,
    author = {{Waelkens}, C. and {Lamers}, H.~J.~G.~L.~M. and {Waters}, L.~B.~F.~M. and 
        {Rufener}, F. and {Trams}, N.~R. and {Le Bertre}, T. and {Ferlet}, R. and 
        {Vidal-Madjar}, A.},
    title = "{Variability of the post-AGB star HR 4049 - Dust obscuration in a binary system}",
    journal = {\aap},
    year = 1991,
    month = feb,
    volume = 242,
    pages = {433-442},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...242..433W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1991A&A...251..495W,
    author = {{Waelkens}, C. and {Van Winckel}, H. and {Bogaert}, E. and {Trams}, N.~R.
        },
    title = "{HD 52961 - an extremely metal-deficient, CNO- and S-rich, pulsating star embedded in a dust cloud}",
    journal = {\aap},
    year = 1991,
    month = nov,
    volume = 251,
    pages = {495-504},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...251..495W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1992A&A...256L..15W,
    author = {{Waelkens}, C. and {Van Winckel}, H. and {Trams}, N.~R. and 
        {Waters}, L.~B.~F.~M.},
    title = "{High-resolution spectroscopy of the central star of the Red-Rectangle nebula}",
    journal = {\aap},
    year = 1992,
    month = mar,
    volume = 256,
    pages = {L15-L18},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...256L..15W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{1993lhls.work..219W,
    author = {{Waelkens}, C. and {Waters}, L.~B.~F.~M.},
    title = "{Binarity of High-Latitude Supergiants - Observational Evidence}",
    booktitle = {ASP Conf. Ser.  45: Luminous High-Latitude Stars},
    year = 1993,
    pages = {219-+},
    adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993lhls.work..219W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1995Ap&SS.224..357W,
    author = {{Waelkens}, C. and {Waters}, L.~B.~F.~M. and {Van Winckel}, H. and 
        {Daems}, K.},
    title = "{Circumstellar Absorption and Emission in the Post-AGB Stars HR4049 and HD213985}",
    journal = {\apss},
    year = 1995,
    month = feb,
    volume = 224,
    pages = {357-360},
    adsurl = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1995Ap%26SS.224..357W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{1996A&A...314L..17W,
    author = {{Waelkens}, C. and {Van Winckel}, H. and {Waters}, L.~B.~F.~M. and 
        {Bakker}, E.~J.},
    title = "{Variability and nature of the binary in the Red Rectangle nebula.}",
    journal = {\aap},
    year = 1996,
    month = oct,
    volume = 314,
    pages = {L17-LL20},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996A%26A...314L..17W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

